Towards Automated Melanoma Screening: Proper Computer Vision & Reliable Results

In this paper we survey, analyze and criticize current art on automated melanoma screening, reimplementing a baseline technique, and proposing two novel ones. Melanoma, although highly curable when detected early, ends as one of the most dangerous types of cancer, due to delayed diagnosis and treatment. Its incidence is soaring, much faster than the number of trained professionals able to diagnose it. Automated screening appears as an alternative to make the most of those professionals, focusing their time on the patients at risk while safely discharging the other patients. However, the potential of automated melanoma diagnosis is currently unfulfilled, due to the emphasis of current literature on outdated computer vision models. Even more problematic is the irreproducibility of current art. We show how streamlined pipelines based upon current Computer Vision outperform conventional models - a model based on an advanced bags of words reaches an AUC of 84.6%, and a model based on deep neural networks reaches 89.3%, while the baseline (a classical bag of words) stays at 81.2%. We also initiate a dialog to improve reproducibility in our community

==> 02a_table_old.tex <==
\begin{sidewaystable*}
\begin{center}
\begin{footnotesize}
%\begin{threeparttable}
	\caption{Summary of literature on melanoma screening, revealing the preference for conservative Computer Vision techniques. We only included works on lesion classification. Detailed discussion in the text.}%\vspace{-0.5cm}}
    \label{tab:SOTA}
    \begin{tabular}{m{2.6cm}lcm{6.05cm}m{1.9cm}m{1.8cm}m{1.6cm}lcm{2.7cm}}
    \toprule
    %\multirow{3}{*}{\textbf{Reference}} & \multirow{3}{*}{\textbf{Year}} & \textbf{Method} & & & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{2}{c}{\multirow{3}{*}{\textbf{Result (\%)}}}  \\ 
    %                                \cmidrule(lr{1em}){4-6} & Low level & Mid level & High level & \textbf{pos~/~neg}  & & \vspace{0.075cm}\\ 
    \multirow{2}{*}{\textbf{Reference}}               & \multirow{2}{*}{\textbf{Year}} & \multirow{2}{*}{\textbf{Seg.?}} & \multirow{2}{*}{\textbf{Low level}} & \multirow{2}{*}{\textbf{Mid level}} & \multirow{2}{*}{\textbf{High level}} & \textbf{Medical} & \textbf{~Dataset} & \multirow{2}{*}{\textbf{Atlas?}} & \multirow{2}{*}{\textbf{Result (\%)}} \\ 
     & & & & & & \textbf{justification} & \textbf{~pos~/~neg}  \\ \midrule
	\toprule
	\multirow{1}{*}{\citet{iyatomi08Computerized}}    & 2008 & $\checkmark$ & Color-, symmetry-, border- and texture-based features & &  ANN & ABCD & \multirow{1}{*}{~198~/~1060} & & SE = 85.9; SP = 86.0; AUC = 92.8 \\ \midrule
	\multirow{1}{*}{\citet{situ08EMBC}}               & 2008 & $\checkmark$ & Wavelets; Gabor-like filters & Classical BoVW  & SVM &  & \multirow{1}{*}{~~30~/~70~~} & &  AUC = 82.2 \\ \midrule
	\multirow{1}{*}{\citet{diLeo10HICSS}}           & 2010 & $\checkmark$ & 2D color histogram; Median filter; Fourier analysis of the grey-level image; & & Decision Tree & 7-point & \multirow{1}{*}{~~~~300~~} & $\checkmark$ &  SE $>$ 85.0; SP $>$ 85.0 \\ \midrule 
	\multirow{1}{*}{\citet{wadhawan11EMBC}}           & 2011 & $\checkmark$ & Color histogram; LBP; Haar Wavelet & & SVM & 7-point & \multirow{1}{*}{~110~/~237~} & $\checkmark$ & SE = 87.3; SP = 71.3 \\ \midrule %ACC: 76.4
	\multirow{1}{*}{\citet{capdehourat11PRL}}           & 2011 & $\checkmark$ & 57 features of shape, color and texture information & & AdaBoost with C4.5 decision\textcolor{white}{aa} trees & ABCD; 7-point & \multirow{1}{*}{~111~/~544~} & & SE = 90.0; SP = 77.0 \\ \midrule 
	\multirow{1}{*}{\citet{wadhawan11ISBI}}           & 2011 & $\checkmark$ & Haar wavelet transform by computing statistical measures (mean and standard deviation) & Classical BoVW & SVM & Menzies; 7-point & ~388~/~912~ & $\checkmark$ & SE = 80.8; SP = 85.6; AUC = 91.1 \\ \midrule
	\multirow{1}{*}{\citet{abbas12Skin}}              & 2012 & $\checkmark$ & Asymmetry, border quantification, color, and differential structure features  & & SVM  & ABCD & \multirow{1}{*}{~~60~/~60~~} & $\checkmark$ & SE = 88.2; SP = 91.3; AUC = 88.0\\ \midrule
	\multirow{1}{*}{\citet{doukas12EMBC}}             & 2012 & $\checkmark$ & Texture (e.g. ASM and GMSM), size (e.g. area, perimeter), asymmetry index and color features & & SVM & & ~800~/~2200 & & ACC = 85.0-90.0 \\ \midrule
	\multirow{1}{*}{\citet{marques12EMBC}}            & 2012 & $\checkmark$ & Color histogram for the RGB, HSV and L*a*b* color spaces; Histograms of gradient magnitude and phase as texture descriptors & & Not provided & & \multirow{1}{*}{~~17~/~146~} & & SE = 94.1; SP = 77.4 \\ \midrule %ACC: 79.1
	\multirow{1}{*}{\citet{mikos12BIOMEP}}            & 2012 & & 12 texture features, the first 3 from the first order statistics (mean value, standard deviation, skewness and kurtosis), and the remaining 8 from GLCM & & Probabilistic Neural Network & & \multirow{1}{*}{~~42~/~88~~} & & ACC = 69.5 \\ \midrule
	\multirow{1}{*}{\citet{barata13iciar}}            & 2013 & $\checkmark$ & Color histograms and moments (mean, standard deviation and skewness); GLCM, Gabor Filters, Laws Masks and Gradient & Classical BoVW & k-NN & & \multirow{1}{*}{~~25~/~151~} & $\checkmark$ & SE = 93.0; SP = 85.0   \\ \midrule
	\multirow{1}{*}{\citet{abuzaghleh2014automated}}  & 2014 & $\checkmark$ & 2-D FFT features; 2-D DCT features; size and complexity features & & SVM & & \multirow{1}{*}{~~40~/~160~} & & ACC = 97.7 \\ \midrule   %ACC: 90.6 
	\multirow{1}{*}{\citet{barata2014two}}            & 2014 & $\checkmark$ & Gradient histograms; Color histograms (RGB, CIE La*b*, L*uv, Opp, HSV and HSI); & Classical BoVW & SVM; k-NN;\textcolor{white}{aa} AdaBoost & ABCD & \multirow{1}{*}{~~25~/~151~} & & SE = 100; SP = 75.0 \\ \midrule
	\multirow{1}{*}{\citet{barata2015improving}}      & 2015 & $\checkmark$ & SIFT; 1-D RGB histograms & Classical BoVW & kNN; SVM & ABCD & \multirow{1}{*}{~241~/~241~} & &  SE = 79.7; SP = 76.0; \\ \midrule
	\multirow{1}{*}{\citet{abedini2015generalized}}   & 2015 & $\checkmark$ & Color, edge, and color LBP histograms & Classical BoVW & SVM & & \multirow{1}{*}{~~40~/~160~} & & SE = 90.0; SP = 90.0 \\ \midrule
	\multirow{1}{*}{\citet{ohki2015building}}         & 2015 & $\checkmark$ & Top 24 features among 120 color image features & & Random Forest & ABCD & \multirow{1}{*}{~168~/~980~} & & SE = 79.8; SP = 80.7 \\ \midrule
    \multirow{1}{*}{\citet{masood2015self}}         & 2015 & $\checkmark$ & Texture features applying autoregressive modeling, GLCM and Fuzzy-Mutual Information based Wavelet transform & & DNN; SVM &  & \multirow{1}{*}{~120~/~170~} & & SE = 90.0; SP = 88.3; ACC = 89.0 \\ \midrule
	\multirow{1}{*}{\citet{codella2015deep}}         & 2015 & & CNN features extracted with a pretrained model from the ILSVRC 2012 & BoVW with\textcolor{white}{aaaa} sparse coding & SVM &  & \multirow{1}{*}{~334~/~2146~} & & SE = 94.9; SP = 92.8; ACC = 93.1 \\ \midrule
	Premaladha and\textcolor{white}{aaaaaa} Ravichandran \citep{premaladha2016novel}     & 2016 & $\checkmark$ & Statistical (e.g. mean, variance, correlation) and shape features (e.g. area, perimeter, asymmetry index) &  & DNN; Hybrid\textcolor{white}{aa} AdaBoost &  & \multirow{1}{*}{~~~~~992~~} & & ACC = 92.9 \\ 
    \bottomrule
    \end{tabular}
\vspace{0.1cm}\\
% | AUC: area under the ROC curve | SE: sensitivity | SP:  specificity
    \begin{tablenotes}
    \centering
    \item ACC: accuracy  |  AUC: area under the ROC curve	| SE: sensitivity | SP:  specificity  
    \end{tablenotes}
    %\end{threeparttable}
\end{footnotesize}
\end{center}
\end{sidewaystable*}

